Balancing Accuracy and Efficiency in Multi-Turn Intent Classification for LLM-Powered Dialog Systems in Production

Accurate multi-turn intent classification is essential for advancing conversational AI systems. However, challenges such as the scarcity of comprehensive datasets and the complexity of contextual dependencies across dialogue turns hinder progress. This paper presents two novel approaches leveraging Large Language Models (LLMs) to enhance scalability and reduce latency in production dialogue systems. First, we introduce Symbol Tuning, which simplifies intent labels to reduce task complexity and improve performance in multi-turn dialogues. Second, we propose C-LARA (Consistency-aware, Linguistics Adaptive Retrieval Augmentation), a framework that employs LLMs for data augmentation and pseudo-labeling to generate synthetic multi-turn dialogues. These enriched datasets are used to fine-tune a small, efficient model suitable for deployment. Experiments conducted on multilingual dialogue datasets demonstrate significant improvements in classification accuracy and resource efficiency. Our methods enhance multi-turn intent classification accuracy by 5.09%, reduce annotation costs by 40%, and enable scalable deployment in low-resource multilingual industrial systems, highlighting their practicality and impact.

==> sections/_outline.tex <==
% \section{Outline}



% problem formulation
% - same as LARA


% Contribution

% experiment1
% - inspiration: high performance in short intent names
% - (Many) shortening intent leads to better performance
% - further investigation (?)
% - sensitivity analysis on length (?)
% - math modelling formula
% - symbolic tuning: label cannot be too long, but cannot have no meaning

% experiment2
% - multi-turn data augmentation pipeline by LARA
% - apply a multi-turn classification pipeline into data augmentation pipeline (LARA)
% - added self-consistency 
% - use pseudo-labelling unsupervised data for small supervised intent classification model, outperform the standard LARA pipeline, reduced latency (RT) 

% 3. in production
% Propose an auto-training framework to update intent classification model to improve operation efficiency 
% business unit with a few clicks use LARA to update model 

==> sections/ack.tex <==
\section{Acknowledgement}
